Self-supervised arbitrary scale super-resolution framework for anisotropic MRI

In this paper, we propose an efficient self-supervised arbitrary-scale super-resolution (SR) framework to reconstruct isotropic magnetic resonance (MR) images from anisotropic MRI inputs without involving external training data. The proposed framework builds a training dataset using in-the-wild anisotropic MR volumes with arbitrary image resolution. We then formulate the 3D volume SR task as a SR problem for 2D image slices. The anisotropic volume's high-resolution (HR) plane is used to build the HR-LR image pairs for model training. We further adapt the implicit neural representation (INR) network to implement the 2D arbitrary-scale image SR model. Finally, we leverage the well-trained proposed model to up-sample the 2D LR plane extracted from the anisotropic MR volumes to their HR views. The isotropic MR volumes thus can be reconstructed by stacking and averaging the generated HR slices. Our proposed framework has two major advantages: (1) It only involves the arbitrary-resolution anisotropic MR volumes, which greatly improves the model practicality in real MR imaging scenarios (e.g., clinical brain image acquisition); (2) The INR-based SR model enables arbitrary-scale image SR from the arbitrary-resolution input image, which significantly improves model training efficiency. We perform experiments on a simulated public adult brain dataset and a real collected 7T brain dataset. The results indicate that our current framework greatly outperforms two well-known self-supervised models for anisotropic MR image SR tasks.

==> table_time.tex <==
\begin{table}[ht]
    \centering
    \resizebox{0.48\textwidth}{!}{
    \begin{tabular}{c|ccc}
        \textbf{Experiment} & \textbf{SMORE}  & \textbf{IREM}          & \textbf{Arssr}  \\ \hline
        \multirow{5}{*}{\textbf{simulation experiment} \cite{hcp}} 
        & Sub \#1   & $1.4\times0.7\times0.7$       & $130\times260\times260$ \\ 
        & Sub \#2   & $0.7\times1.75\times0.7$      & $260\times104\times260$ \\  
        & Sub \#3   & $0.7\times0.7\times2.1$       & $260\times260\times87$  \\ 
        & Sub \#4   & $2.45\times0.7\times0.7$      & $74\times260\times260$  \\ 
        & Sub \#5   & $0.7\times2.8\times0.7$       & $260\times65\times260$  \\ \hline
        \multirow{2}{*}{\textbf{real experiment}}    
        & Fetus \#1 & $1\times0.2\times0.2$         & $45\times225\times225$  \\ 
        & Fetus \#2 & $1.1\times0.1953\times0.1953$ & $54\times432\times432$  \\
    \end{tabular}}
    \caption{Details of the two datasets used in our experiments.}
    \label{tab:data}
\end{table}
